The Gambler's Ruin Problem and Quantum Measurement

The dynamics of a single microscopic or mesoscopic non quantum system interacting with a macroscopic environment is generally stochastic. In the same way, the reduced density operator of a single quantum system interacting with a macroscopic environment is a priori a stochastic variable, and decoherence describes only the average dynamics of this variable, not its fluctuations. It is shown that a general unbiased quantum measurement can be reformulated as a gambler's ruin problem where the game is a martingale. Born's rule then appears as a direct consequence of the optional stopping theorem for martingales. Explicit computations are worked out in detail on a specific simple example.

==> eptcsdata.tex <==
\providecommand{\firstpage}{100}
\providecommand{\publicationstatus}{G. Di Molfetta, V. Kendon \& Y. Shikano (Eds.): 9th International\\ Conference on Quantum Simulation and Quantum Walks (QSQW 2020)\\
EPTCS 315, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.315.10}{10.4204/EPTCS.315.10}}

